Two-dimensional quantum dilaton gravity and the quantized cosmological constant

The cosmological constant problem is one of the long-standing issues of modern physics. While we can measure the value of the cosmological constant with great accuracy, we are not able to calculate it in a coherent theoretical framework. On the contrary the theoretical predictions in Quantum Field Theory are radically different from observations. This disagreement is a hint of the difficult conciliation of Quantum Mechanics and General Relativity in a theory of Quantum Gravity. Current approaches to the cosmological constant problem, in particular, do not account for the quantum nature of the gravitational interaction and rely on perturbative calculations. In this thesis we address the issue in the simplified framework of two-dimensional dilaton-Maxwell gravity, coupled to scalar matter fields. In this setting we are able to quantize our model non-perturbatively in Dirac's approach to constrained systems. We determine that the realization of the classical symmetries at the quantum level provides a mechanism that fixes the value of the cosmological constant once a specific quantum state of the Universe is selected. Furthermore Quantum Gravity introduces opposite contributions to the cosmological constant, admitting a range of values compatible with current observations.

==> files/central_charge_ghosts.tex <==
\begin{eqnarray*}
&\left[L_{r}^{+},L_{q}^{+}\right]=\\=&\sum_{n}\sum_{m}\left(q+m\right)\left(r+n\right)\left(c_{n}b^{r-n}c_{m}b^{q-m}-c_{m}b^{q-m}c_{n}b^{r-n}\right)\times\\&\times e^{-\epsilon\left(|n|+|r-n|+|m|+|q-m|\right)}=\\=&\sum_{n}\hbar\left(q-r+n\right)\left(r+n\right)c_{n}b^{r+q-n}e^{-\epsilon\left(|n|+2|r-n|+|q+r-n|\right)}-\\&-\sum_{n}\hbar\left(q+n\right)\left(r+n-q\right)c_{n}b^{r+q-n}e^{-\epsilon\left(2|n-q|+|r+q-n|+|n|\right)}=\\=&\hbar\sum_{n}c_{n}b^{r+q-n}e^{-\epsilon\left(|n|+|q+r-n|\right)}\times\\&\times\left(\left(q-r+n\right)\left(r+n\right)e^{-\epsilon2|r-n|}-\left(q+n\right)\left(r+n-q\right)e^{-\epsilon2|n-q|}\right)
\end{eqnarray*}
By assuming that $r+q>0$, we have:
\begin{eqnarray*}
=&\hbar\sum_{n<r+q}c_{n}b^{r+q-n}e^{-\epsilon\left(|n|+|q+r-n|\right)}\left(\left(q-r+n\right)\left(r+n\right)e^{-\epsilon2|r-n|}-\left(q+n\right)\left(r+n-q\right)e^{-\epsilon2|n-q|}\right)+\\&\qquad-\hbar\sum_{n\ge r+q}b^{r+q-n}c_{n}e^{-\epsilon\left(|n|+|q+r-n|\right)}\left(\left(q-r+n\right)\left(r+n\right)e^{-\epsilon2|r-n|}-\left(q+n\right)\left(r+n-q\right)e^{-\epsilon2|n-q|}\right)+\\&\qquad+\hbar^{2}\delta_{r+q}\sum_{n\ge0}e^{-\epsilon2n}\left(\left(-2r+n\right)\left(r+n\right)e^{-\epsilon2|r-n|}-\left(-r+n\right)\left(2r+n\right)e^{-\epsilon2|n+r|}\right)=
\end{eqnarray*}

==> files/discussion.tex <==
We have seen that in the case of two-dimensional dilaton-Maxwell gravity, and in particular for the subclass of model which admit a dual description in terms of Liouville fields, the realization of the classical symmetry at the quantum level provides a mechanism that fixes the cosmological constant to a specific value once a particular quantum state is required to be physical. In this approach $\Lambda$ is considered a free parameter which can be fixed by consistency conditions determined by quantum gravity.\\
The value of $\Lambda$ includes classical and quantum contributions and it is determined in a fully non-perturbative quantum theory of gravity and scalar matter. To this respect this result takes full advantage of the lower dimensional setting: the usual computation of the value of the cosmological constant is performed only considering one-loop contributions of matter and gauge fields in perturbation theory in a flat background geometry.\\
Turning the physicality conditions for quantum states, \emph{i.e.} annihilation by the action of the quantum constraints, into equations for $\Lambda$ we can account for the quantum vacuum fluctuations and the excitations of the quantum fields. In particular we can see that, in contrast with the positive contributions of the matter fields, one of the gravitational degrees of freedom provides with a negative one, therefore allowing for partial cancellations and small values of $\Lambda$ even in the presence of matter fields.\\
Dispite the technical simplifications of the lower number of dimensions however it is not easy to freely study the case of arbitrarily high excitations and/or arbitrarily many matter fieds: an expression for $\Lambda$ in terms of occupation numbers and complex coefficients of the quantum states of the fields has to be obtained from imposing the Fourier modes of \eqref{qc1} and \eqref{qc2} to vanish. This keeps us from determining a general formula for the cosmological constant and we are forced to do it on a case by case way and we limited our study to the lower excitations only.\\
In our approach, considering the way we exploited the realization of the quantum constraints, we are able to determine, for a given quantum state of our Universe, which is the value that the cosmological constant has to take. In this way it is natural to study the spectrum of values of $\Lambda$ for particular subsets of quantum states. We can then see a parallel with the principles behind the landscape of string theory. In both cases there is a countable set of configurations (the $10^{500}$ vacua VS. the infinitely many quantum states) and for each of them there is a specific value for the cosmological constant. In neither cases we know a priori which one is the configuration we are in. Let us stress however that in our case, albeit two-dimensional, we are not introducing new physics but simply quantizing a theory of gravity and matter.\\
While the techniques applied in this work are especially two-dimensional, the results have a more general significance. As discussed in Section \ref{sec:ccinqg} the classical constaints which appear in the canonical formulation of any diffeomorphism invariant theory can be exploited in the quantum theory to determine the cosmological constant required for a given quantum state to be physical. We can therefore expect similar results in dimensions higher than two: in particular in the limit in which quantum gravity reduces to General Relativity we should be able to see the cosmological constant as made up by classical contributions and quantum corrections, as it is the case in our discussion.\\
A brief remark can be done on Spherically Reduced Gravity, which is a particular model included in the general dilaton-Gravity action. It has to be said that SRG is not one of the models which allows for a dual description in terms of decoupled Liouville fields. If no alternative decoupled formulation is accessible the only possibility is to proceed perturbatively, possibly employing the path integral approach, as developed in the literature (\cite{Grumiller:2002nm} and references therein). The dilaton field $X$ in SRG is related to the anglular dynamics of four-dimensional General Relativity. On the other hand in our decoupled model the $Z$ and $Y$ fields can be roughly related to the conformal mode $\varphi$ and the dilaton $X$, respectively. We can then say that it is the conformal mode to contribute negatively to $\Lambda$, while the dilaton contributes in a way similiar to a matter field. We can therefore speculate that in a four-dimensional (roughly spherically symmetric) scenario excitations of the conformal mode might provide cancellations that would allow for a small value of the cosmological constant in the same way that it happens in two-dimensions.
